Elementare Zahlentheorie

This is a textbook about elementary number theory, with emphasis on classical topics around the Euklidean Algorithm.

==> Tabelle_L03_A.tex <==
% Die Tabelle aus der Aufgabe 3.3
\begin{center}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c||c|} \hline
		~~$j$~~  & \rule{0pt}{2.7ex}   ~~$a_j$~~   &  ~~$b_j$~~  &  ~~$c_j$~~ &  ~~$q_j$~~  & ~~$x_j$~~   &  ~~$a_j^*$~~   &  ~~$b_j^*$~~   &  ~~$c_j^*$~~  & ~~$x_j^*=x_j-q_j$~~   \\[0.3em] \hline \hline
		
		0  &   14   &  -20  &   7 &  0   &\rule{0pt}{3.5ex} $\frac{\sqrt{8}+20}{28}$     &  14   &  -20   &  7    &  $\frac{\sqrt{8}+20}{28}$ \\[0.3em] \hline %\hline
		
		1  &  -7    &  20   &  -14  &   1  &  \rule{0pt}{3.5ex}   $\frac{\sqrt{8}-20}{-14}$      &  -7    &  6   &  -1     &    $\frac{\sqrt{8}-6}{-14}$   \\[0.3em] \hline %\hline
		
		2      &  1    &  -6   &  7  &   4  &\rule{0pt}{3.5ex}    $\frac{\sqrt{8}+6}{2}$   &  1    &  2   &  -1   &  $\frac{\sqrt{8}-2}{2}$   \\[0.3em] \hline %\hline
		
		3      &  1    &  -2   &  -1  &  2  & \rule{0pt}{3.5ex}   $\frac{\sqrt{8}+2}{2}$   &  1    &  2   &  -1  
		&  $\frac{\sqrt{8}-2}{2}$  \\[0.3em] \hline
	\end{tabular}
\end{center}




